The Possibility Problem for Probabilistic XML (Extended Version)

We consider the possibility problem of determining if a document is a possible world of a probabilistic document, in the setting of probabilistic XML. This basic question is a special case of query answering or tree automata evaluation, but it has specific practical uses, such as checking whether an user-provided probabilistic document outcome is possible or sufficiently likely. In this paper, we study the complexity of the possibility problem for probabilistic XML models of varying expressiveness. We show that the decision problem is often tractable in the absence of long-distance dependencies, but that its computation variant is intractable on unordered documents. We also introduce an explicit matches variant to generalize practical situations where node labels are unambiguous; this ensures tractability of the possibility problem, even under long-distance dependencies, provided event conjunctions are disallowed. Our results entirely classify the tractability boundary over all considered problem variants.

==> old.tex <==

\section{Hardness of POSS for fie and cie}

\begin{proposition}
If we allow edges to be labeled by arbitrary conjunctions of independent events,
then the POSS problem is hard (NP-hard for computation, \#P-hard for counting)
in all possible formulations, even when $D$ has only one node and $W$ has height
2.
\end{proposition}

\begin{proof}
  Consider a trivial possible world and branches: probability for all branches
  to not be there: conjunctions of negations of conjunctions.
\end{proof}

\todo{What about conjunctions of positive events only?}

\section{Tractability under the unique match assumption}

\todo{Formally define the unique match assumption and sufficient conditions for
it to hold.}

\todo{Define formally independent atomic events. Can it be made to encode mux?
(non-boolean values?)}

\begin{proposition}
If we assume that $W$ has a unique match in $D$, then all
formulations of the problem can be solved in PTIME.
\end{proposition}

\begin{proof}
  Worst case is independent atomic events, or mux (what about mux and det?).
  Consider the match. If order constraints hold, check if the match satisfies
  them. Collect the conditions as a large conjunction, and the conditions on the
  rest of the document to make it disappear. See if this conjunction is
  contradictory or not; compute its probability if requested.

  \todo{Should be possible to adapt this to multiple matches (polynomial number of
  them) by accounting all cojunctions; must be careful not to count multiple
times when the acceptable assignments overlap (but should be doable).}
\end{proof}

\section{Hardness of the computation variant}

\begin{proposition}
  Without the unique match assumption, on unordered documents, the computation
  version of POSS is \#P-hard, even with just mux or just ind, even with
  probabilities of just 1/2, even on documents of bounded height.
\end{proposition}

\begin{proof}
  By reduction from the problem of computing the number of perfect matches in a
  bipartite graph.
\end{proof}

This shows hardness for partial orders too.

\todo{What about total orders? it's probably still hard, but how to reduce? no
in fact think it can be done dynamically}

\section{Hardness of the partially ordered variant}

\begin{proposition}
  Without the unique match assumption, for partially ordered $D$ and $W$, the
  decision version of POSS is NP-hard, even when the order of $W$ is total and
  the order of $D$ is of order dimension 2, even on documents of bounded height.
\end{proposition}

\begin{proof}
  From unary-3-partition, like in the provenance paper.
\end{proof}

\section{Hardness of long-distance}

Considering the possible world $a b ... c$ and the probabilistic document $a a
... a, ..., z z ... z$ labeled with individual positive events, POSS asks for a
subset of events intersecting the set of events of the $a$'s, $b$'s, etc.,
exactly once, aka, exact hitting set or exact set cover. This is NP-hard, and
the presence or absence of order is irrelevant.

\todo{What about the counting formulation?}

\section{Tractability of the independent uncertainty models}

\begin{proposition}
  Without the unique match assumption, for totally ordered or for unordered $D$
  and $W$, the decision version of POSS can be solved in PTIME.
\end{proposition}
  
\begin{proof}
  In the ordered case: recursive dynamic algorithm related to the dynamic
  algorithm of the provenance paper. Must also ask whether subtrees can match,
  must match, can be absent. I think it would work.

  In the unordered case: perfect matching problem, maybe adding empty nodes to
  force elements to be missing.
\end{proof}

